Optimizing Static Linear Feedback: Gradient Method

The linear quadratic regulator is the fundamental problem of optimal control. Its state feedback version was set and solved in the early 1960s. However the static output feedback problem has no explicit-form solution. It is suggested to look at both of them from another point of view as matrix optimization problems, where the variable is a feedback matrix gain. The properties of such a function are investigated, it turns out to be smooth, but not convex, with possible non-connected domain. Nevertheless, the gradient method for it with the special step-size choice converges to the optimal solution in the state feedback case and to a stationary point in the output feedback case. The results can be extended for the general framework of unconstrained optimization and for reduced gradient method for minimization with equality-type constraints.

==> Optimizing Static Linear Feedback_ Gradient Method (revised)/main_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi
\usepackage{algorithmic} % <- Preamble
\Crefname{ALC@unique}{Line}{Lines} % <- Preamble
% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamthm{problem}{Problem}
\newsiamthm{example}{Example}
%\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
%\headers{Optimizing Static Linear Feedback: Gradient Method}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.

\title{Optimizing Static Linear Feedback: Gradient Method\thanks{Submitted to the editors on April 2020. \funding{The revised version of this work was funded by Russian Science Foundation under Grant 21-71-30005.}}}

% Authors: full names plus addresses.
\author{Ilyas Fatkhullin${}^\ddagger$\thanks{Moscow Institute of Physics and Technology, Institutskiy per. 9, 141700, Moscow Region, Dolgoprudny, Russia (\email{ilyas.fn979@gmail.com}).}%$\ddagger$ 
\and Boris Polyak\thanks{Institute for Control Sciences, Profsoyuznaya 65, 117806, Moscow, Russia
  (\email{boris@ipu.ru}).}
  }

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

